Repairing Conflicts among MVCC Transactions

The optimistic variants of MVCC (Multi-Version Concurrency Control) avoid blocking concurrent transactions at the cost of having a validation phase. Upon failure in the validation phase, the transaction is usually aborted and restarted from scratch. The "abort and restart" approach becomes a performance bottleneck for the use cases with high contention objects or long running transactions. In addition, restarting from scratch creates a negative feedback loop in the system, because the system incurs additional overhead that may create even further conflicts. In this paper, we propose a novel approach for conflict resolution in MVCC for in-memory databases. This low overhead approach summarizes the transaction programs in the form of a dependency graph. The dependency graph also contains the constructs used in the validation phase of the MVCC algorithm. Then, in the case of encountering conflicts among transactions, the conflict locations in the program are quickly detected, and the conflicting transactions are partially re-executed. This approach maximizes the reuse of the computations done in the initial execution round, and increases the transaction processing throughput.

==> problem.tex <==

\section{The Problem: Costly Restarts} \label{sec:problem}
\SBJ{-----NOT REALLY IMPORTANT..TOO MUCH CONTENT-----}


\SBJ{----------------------------------------------------------------------------------------------------}

In addition, the increasing tendency to use in-memory databases for transaction processing due to the decreased costs of DRAM \cite{larson11} has led to new research directions in this area. Most classical scheduling algorithms in the literature were initially proposed for disk-based databases. Thus, some research effort was required and done to find the best concurrency control techniques for in-memory databases, and fitting them against the new constraints in this environment.

%In the rich literature on transaction processing and concurrency control algorithms, the research has been focused mostly on finding algorithms for detecting or preventing conflicts. However, when a conflict happens, the common solution is always to abort and restart, unless nested transaction model is being used. The questions addressed in this paper are: \emph{How to avoid abort and restart upon conflicts (without explicitly using nested transactions)? Can we find an approach that has reasonable overhead and which allows us to reuse the computation done during the initial execution of a conflicted transaction, and use it for either compensating the conflict, or faster re-execution of the transaction?}

%Such a solution, if it exists, only matters if the number of transactions that are conflicting is high. The two factors that contribute the most to an increase in the number of conflicts are : (1) having high contention data objects (that will be read and updated by several concurrent transactions), and (2) having long running transactions (lifespan of which intersects with that of many other transactions). %\cite{xxxx}. SHOULD NOT WE CITE SOMETHING HERE?!

%Consequently, the possible solution for conflict resolution is beneficial for these cases. On the other hand, one could propose  pessimistic concurrency control algorithms for such cases. However, we should notice that, firstly, a pessimistic approach to concurrency control would yield bad performance for long running transactions (as acquiring a highly demanded resource by a long running transaction means stopping almost all other transactions). Secondly, general DBMSs normally implement a specific concurrency control technique and are optimized for that technique.  Using a pessimistic algorithm might not be available as an option. 

%The state-of-the-art research proposes an optimistic \MVCC algorithm as the best fit for concurrency control in in-memory databases \cite{neumann15}. This algorithm is referred by \NMVCC throughout the rest of this paper, where \NMVCCInitials stands for the first author's initial. In the next section we propose our solution which is built on top of \NMVCC, adding conflict resolution to it.

%\SBJ{one sentence about semantic stuff.. closure}

